On the Approximability of Geometric and Geographic Generalization and the Min-Max Bin Covering Problem

We study the problem of abstracting a table of data about individuals so that no selection query can identify fewer than k individuals. We show that it is impossible to achieve arbitrarily good polynomial-time approximations for a number of natural variations of the generalization technique, unless P = NP, even when the table has only a single quasi-identifying attribute that represents a geographic or unordered attribute: Zip-codes: nodes of a planar graph generalized into connected subgraphs GPS coordinates: points in R2 generalized into non-overlapping rectangles Unordered data: text labels that can be grouped arbitrarily. In addition to impossibility results, we provide approximation algorithms for these difficult single-attribute generalization problems, which, of course, apply to multiple-attribute instances with one that is quasi-identifying. We show theoretically and experimentally that our approximation algorithms can come reasonably close to optimal solutions. Incidentally, the generalization problem for unordered data can be viewed as a novel type of bin packing problem--min-max bin covering--which may be of independent interest.

==> binpack.tex <==
\subsection{The Min-Max Bin Covering Problem}

Consider the following problem, which we call the
{\sl Min-Max Bin Covering Problem}.

\begin{list}{}{}
\item
Input: Positive integers $x_1,x_2,\ldots,x_n$  
and a positive integer nominal bin capacity $k$.
\item
Output: a partition of $\{1,2,\ldots,n\}$ into subsets $S_j$,
satisfying the constraint that for each $j$, 
\begin{equation} \label{gl:constraint}
\sum_{i\in S_j} x_i \ge k,
\end{equation}
and minimizing the objective function 
\begin{equation} \label{gl:objective}
\max_j \sum_{i\in S_j} x_i.
\end{equation}
\end{list}

\noindent We will say that a partition satisfying (\ref{gl:constraint})
for all $j$ is {\sl feasible}, and that the function shown in
(\ref{gl:objective}) is the {\sl cost} of this partition.  Note that
any feasible solution has cost at least $k$.  Note also that if
$\sum_{i=1}^n x_i < k$, there is no feasible solution; we will therefore
restrict our attention to instances for which
\begin{equation} \label{gl:assume.feasible}
\sum_{i=1}^n x_i \ge k.
\end{equation}
We will sometimes
use terminology from bin packing.  Thus we may refer to a partition 
of the items as a packing, 
a set $S_j$ in the partition as a bin,
and $\sum_{i\in S_j}x_i$ as the level to which this bin is packed.

The motivation for this is $k$-anonymization of symbolic data. We assume
that we have a collection of records for which we wish to protect the
privacy, by releasing only aggregate information about sets of at
least $k$ records per set. Certain pairs of records must be included in
the same set as each other (perhaps because they are very similar in
certain fields) and the numbers $x_i$ represent the sizes of the
connected components that must be grouped together.

\begin{theorem} \label{gl:2approxlimit}
If the numbers $x_i$ and the capacity $k$ are given in binary,
it is not possible to approximate the solution to within less than a
factor of 2 in polynomial time unless $P=NP$.
\end{theorem}

\proof: We show that the problem is $NP$-hard by a reduction from
Subset Sum: We are given a list of numbers $x_1, x_2, \ldots, x_n$ and
asked whether it can be divided into two parts each summing exactly
to $\frac{1}{2} \sum_i x_i$.  Given a Subset Sum instance $I$, we
construct a Min-Max Bin Covering instance $I'$ with the same $n$
and $x_i$, and $k=\frac{1}{2} \sum_i x_i$.  If the answer to the given
Subset Sum instance $I$ is yes, the cost of the optimum solution to
the Min-Max Bin Covering instance $I'$ is $k$, which is clearly the
best we can hope for.  If, on the other hand, the answer to the Subset
Sum problem is no, there is no way to partition the items into two or
more subsets each of which has total size at least $k$; thus the only
feasible solution, and hence the optimum, is achieved by putting all
items into a single bin, which has cost $2k$.  Thus an algorithm that
approximates the optimum cost for $I'$ to within a factor better than 2
would have to solve it exactly, and therefore would also solve the
given Subset Sum instance $I$.\qed

If $A$ is some algorithm for Min-Max Bin Covering Problem, and $I$
is some instance, let $A(I)$ denote the cost of the solution obtained
by $A$.  Let $\opt(I)$ denote the optimum cost for this instance.

We will precede name of a problem by ``unary'' to indicate that all
integers in the input are encoded in unary.

\begin{theorem} \label{gl:unary4/3approxlimit}
Assuming $P\ne NP$, there is no polynomial time algorithm
$A$ for unary Min-Max Bin Covering
that guarantees
\begin{equation} \label{gl:Aapproxbound}
A(I) \le r \, \opt(I) + d
\end{equation}
for any fixed $r < 4/3$ and $d$.
\end{theorem}

\proof.  Suppose that we had such an algorithm $A$.
We will show how this could
be used to solve the unary 3-Partition problem (defined below)
in polynomial time; since 3-Partition is strong $NP$-complete
\cite[$NP$-complete problem SP15]{gj-cigtn-79} this would establish that $P=NP$.
In the 3-Partition problem we are
given a set $S$ of $3n'$ weights $w_1,w_2,\ldots,w_{3n'}$,
and a bound $B$, and are assured that
$$\sum_{i=1}^{3n'} w_i = n' B$$
and that each $w_i$ satisfies $B/4 < w_i < B/2$.
We are asked whether we can partition $\{1,2,\ldots,3n'\}$ into $m$ sets $S_j$
such that for each $j$, $\sum_{i\in S_j} w_i = B$.
As noted in \cite{gj-cigtn-79}, if the answer is yes then each $S_j$ must have
cardinality three.

Given an instance $I$ of 3-Partition, choose
an $M$ large enough so that 
\begin{equation} \label{gl:Mdef}
4 M > r (B + 3M) + d;
\end{equation}
note that for fixed $r<4/3$ and $d$ the required $M$ has a value that is
polynomial in the size of $I$.
Form a Min-Max Bin Covering instance $I'$ with $n=3n'$,
$k=B+3M$, and
$x_i = M + w_i$.
If the answer to the given 3-Partition instance is yes, we can find a partition
of $\{1,2,\ldots,3n'\}$ into $m$ subsets $S_j$ such that for each $j$ we have
$|S_j|=3$ and $\sum_{i\in S_j} w_i = B$;
hence each $\sum_{i\in S_j} x_i = B + 3M$.
Thus have $\opt(I') \le B + 3M$, so using (\ref{gl:Aapproxbound}) 
and (\ref{gl:Mdef}) we have
$$A(I') \le r \, \opt(I') + d \le r(B + 3M) + d < 4M.$$
On the other hand, if the answer
is no, we cannot partition $X$ into $m$ subsets each having
total weight at least $B$, so any feasible partition uses at most $m-1$
subsets.  Hence at least one of the subsets has cardinality at least 4,
so $\opt(I')\ge 4M$ and therefore $A(I')\ge 4M$.  Thus by comparing
$A(I')$ to $4M$ we could distinguish yes instances of unary 3-Partition
from no instances.\qed

Having shown lower bounds on the efficient approximability of the
problem, we now turn to polynomial time algorithms that achieve
guaranteed approximations.  A factor of three approximation is
easily obtained.

\begin{theorem} \label{gl:approx3} There always exists a solution with cost
$\max(k - 1 + \max_{x\in S} x_i, 3k-3)$ that can be found in linear time.
\end{theorem}

\proof: Put all items of size $k$ or greater into their own bins, and
greedily partition the remaining items into bins all except possibly the
last of which is filled to a level of at least $k$.
All but the last bin in the greedy partition have level at most $2k-2$,
as they each have level
at most $k-1$ before the last item is added and this last item
has size less than $k$. There may be one leftover bin with level less than
$k$ which must be merged with some other bin, leading to the claimed
bound.\qed

With more effort we can improve this to a factor of 5/2.
For convenience in the remainder of this section, we 
scale the problem by dividing by~$k$.
Thus the bin capacity becomes~1, and the item sizes are multiples of $1/k$.

\begin{lemma}  \label{gl:2part}
Suppose we are given a list of positive
numbers $x_1,x_2,\ldots,x_n$,
with each $x_i\le m$ and $\sum_{i=1}^n x_i = s$.
Then we can partition the list into two sublists
each having a sum of at most $(s+m)/2$.
\end{lemma}

\proof.  Form the partial sums $p_i = \sum_{j=1}^i x_i$,
$i=0,1,\ldots,n$.  Then successive partial sums are clearly at most
$m$ apart, so we can find some $\ell$ so that $(s-m)/2 \le p_\ell \le
(s+m)/2$.  Hence if we cut the list in half just after the $\ell$th
element we will have two sublists summing to at most $(s+m)/2$.\qed

\begin{lemma} \label{gl:3part}
Suppose we are given a list of numbers $x_1,x_2,\ldots,x_n$,
with each $x_i\le 1/2$ and $\sum_{i=1}^n x_i = 1$.
Then we can partition the list into three parts
each having a sum of at most $1/2$.
\end{lemma}

\proof.
For convenience assume the $x_i$ appear in decreasing order.
Let the first sublist contain only $x_1$,
so its sum is clearly at most 1/2.
The remaining list has sum $1-x_1$ and no entries greater than
$x_1$, so by Lemma~\ref{gl:2part} we can partition it into two lists
each having sum at most $(1 - x_i + x_i)/2=1/2$.\qed

\begin{theorem} \label{gl:thm5/2}
There is a polynomial algorithm to solve the {\sl Min-Max Bin Covering Problem}
with an approximation factor of $5/2$.
\end{theorem}

\proof.  We will assume without loss of generality
that no item sizes exceed 1, since we could always pack each such item
in a bin by itself without worsening the approximation ratio.
We will show how to construct in polynomial time a solution that has
cost at most 5/2 times the optimum.

Assume the items are numbered in order of decreasing size.
Pack them greedily in this order into successive bins,
moving to a new bin when we have covered the current bin.  Note that
then all of the bins will be filled to a level
of at most 2, and all of the bins except the last
are filled to a level of at least 1.  If the last bin is also
filled to a level of at least 1, this packing is feasible
and has cost less than 2, so it is within a factor of 2 of the
optimum.

Next suppose that the last bin is filled to a level less than 1.
If we have used only three bins so far, the total size of
all the items is less than 5, so they can cover at most 4 bins; thus
we can start from scratch and 
find the optimum solution in $O(n^4)$ time by exhaustive search.
So assume we have used at least 4 bins.  

Now let $f$ be size of the largest
item in the final bin, and let $r$ be the total size of the other items
in the last bin.  Consider two cases.

Case 1.  $f \le 1/2$.  
Then all items in the last bin are less than $1/2$ 
in size, so by Lemma~\ref{gl:3part} we can partition them into three sets,
each of total size at most 1/2.  Add each of these sets to one of the first
three bins, so no bin is filled to more than 5/2.  (We no longer use the
last bin.)  Thus we have achieved an approximation ratio of 5/2.

Case 2.  $f > 1/2$.  Call an item {\sl large} if its size is greater
than 1/2, and {\sl small} otherwise.  Note that in this case there must
be an odd number of large items, since each bin except the last
has exactly two large items.  Note also that $r$ in this case
is the total size of the small items, and $r<1/2$.

Case 2.1.  $x_1 + r \ge 1$.  Then swap items $x_1$ and $f$, so the
last bin will be filled to a level $x_1 + r \in [1,2]$.
Also, the first bin will contain two items of size in the range [1/2,1]
and thus be filled to a level in the range [1,2].  Thus we have
a solution that meets the constraints and has cost at most 2.

Case 2.2.  $x_1 + r \le 1$.  Since $r$ is the total size of the small
items, if any bin had only one large item it could not be filled to
a level of at least 1 as required for feasibility.  Thus the optimum
solution has no bin containing only one large item.  Since there are an
odd number of large items, this means that the optimum solution has at least
one bin with 3 or more large items, so the cost of the optimum solution
is at least 3/2.  But then since the simple algorithm of 
Theorem~\ref{gl:approx3} gives a solution of cost less than 3, it provides
a solution that is at most twice the optimum. \qed

Note that there is a gap between our lower bound of 2 and our upper bound
of 5/2.  It would be interesting to try do reduce this gap.
Finally, we note that if one is willing to relax the constraints as
well as the cost of the solution obtained, an $\epsilon$-approximation
of sorts is possible.

\begin{theorem} \label{gl:1pluseps}
Assume that all numbers in the input are expressed in binary,
and let $\epsilon > 0$ be a fixed constant.
There is a polynomial time algorithm that, 
given some instance $I$ of Min-Max Bin Covering, 
finds a partition of $\{1,2,\ldots,n\}$ into disjoint subsets $S_j$
such that 
\begin{equation} \label{gl:modconstraint}
\sum_{i\in S_j} x_i \ge 1 - 2 \epsilon,
\end{equation}
and
\begin{equation} \label{gl:modobjective}
\max_j \sum_{i\in S_j} x_i \le \opt(I) + \epsilon
\end{equation}
\end{theorem}

 \proof: We can restrict our attention to problems having all $x_i<1$,
since if there were larger items, we could first solve the
approximation problem formed by omitting them, and
then pack them into separate bins without introducing any violations
of (\ref{gl:modconstraint}) or (\ref{gl:modobjective}).  
With this assumption we know from Theorem~\ref{gl:approx3}
that $\opt(I) \le 3$.

\newcommand{\gltype}{{\rm type}}
The idea of the proof is as follows.  There are of course
exponentially many ways that we might pack the items into bins; we reduce the
number we must consider by putting similar packings into groups,
and considering only the different groups.
We do this as follows.
Call those $x_i$ that are greater than or equal to
$\epsilon$ {\sl large}, and the others {\sl small}.
Let $b=(1-\epsilon)^{-1}\sum_{i=1}^n x_i$; note that
$b\le n/(1-\epsilon)$, and any partition satisfying 
(\ref{gl:modconstraint}) will have at most $b$ bins.
Let $N$ be the largest integer for which $\epsilon(1+\epsilon)^N$
is less than one; note that $N$ is a constant depending only on $\epsilon$.
Let 
$$
\hat S = \bigl\{\epsilon(1+\epsilon)^\ell: \ell \in \{0,1,2,\ldots,N\}\bigr\};
$$
Let the {\sl type} of a packing $P$, written $\gltype(P)$, be the 
result of discarding all small items in $P$, and 
rounding each large $x_i$ to the largest value in $\hat S$
that is less than or equal to $x_i$; we denote this value $\hat x_i$.
For the small items we simply let $\hat x_i=x_i$.
Note that any type can be viewed as
a partial packing of bins using only items from $\hat S$.

Since, for fixed $\epsilon$, there are only a constant number of item
sizes in $\hat S$, and each of these is at least $\epsilon$, there are
only finitely many ways of packing a bin to a level of at most 3 using
the rounded values; call each of these ways a {\sl configuration} of a
bin.  Since the order of bins does not matter, we can represent the
type of a packing by the number of times it uses each configuration.
It is not hard to show that for fixed $\epsilon$, as in the proof
of \cite[Lemma 9.4]{vazirani-aa}, there are only
polynomially many types having at most $b$ bins.  (Of course, for
small $\epsilon$, this will be a polynomial of very high degree.)  We
will allow types that leave some of the bins empty.

Let $P$ be some packing that contains no small items.  Define the {\sl
greedy completion} of $P$ to be the result of starting with with $P$ and then
greedily packing each of the small items into the bin in currently
filled to the lowest level.

Define the {\sl $t$-gap} of a bin to be the maximum of 0 and $t$ minus
the total size of the items in the bin; let the $t$-gap of the entire packing
to be the sum of the $t$-gaps over all bins.
Say a type $T$ is {\sl weakly feasible} if the $(1-\epsilon)$-gap of $T$ is 
less than $s$, 
where $s$ is the total size of the small items.

The algorithm proceeds as follows.  Enumerate all possible types $T$.
Of those that are weakly feasible, select one, say $T^*$, that minimizes
the maximum level to which any bin is packed in the greedy completion
of $T^*$.
Return as the approximate solution the result of replacing 
all large items in the greedy completion, which have values from
$\hat S$, by the corresponding original unrounded values.

We begin the proof of correctness of this algorithm
by showing that it actually does return some packing,
i.e., that it does not reject all types as not weakly feasible.
To see this, note that
by our assumption (\ref{gl:assume.feasible}) there is at least
one feasible packing $P$ for the original problem.
Since $P$ is feasible, we know that if we remove all small items from
$P$ we will have a packing with a 1-gap of at most $s$.  When
we shrink the large items to values in $\hat S$ to obtain
$\gltype(P)$, we
will have a $(1-\epsilon)$-gap of at most $s$, so $\gltype(P)$ is
weakly feasible.

Next we show that the packing computed by the algorithm will satisfy conditions
(\ref{gl:modconstraint}) and (\ref{gl:modobjective}).
Let $P$ be packing produced by the algorithm; 
then we know that $\gltype(P)$ is weakly feasible.
Assume for a contradiction that 
some bin in $P$ is packed to a level of less than $1-2\epsilon$.
Then when we were forming the greedy completion of $\gltype(P)$
none of these small items can have filled a bin to a level beyond $1-\epsilon$,
so each small item $x_i$ we added to the packing
decreases the $(1-\epsilon)$-gap by $x_i$.
Thus the $(1-\epsilon)$-gap of is reduced to $0$, contradicting
our assumption, so the packing computed by the algorithm will satisfy
condition (\ref{gl:modconstraint}).

Finally, we show that the computed packing will satisfy
(\ref{gl:modobjective}).  Let $P^*$ be an optimum packing
for the original problem.  Let $b^*$ be the number of
bins in $P^*$, and let $T=\gltype(P^*)$.
Then $T$ is weakly feasible, so we will consider the greedy completion
$\bar T$ of $T$.
Suppose for a contradiction that some bin in $\bar T$
is packed to a level above $\opt(I)+\epsilon$.  Then since each small
item is at most $\epsilon$ and we are packing greedily it must be that
all bins in $\bar T$ are packed to a level above $\opt(I)$.  Hence
we must have $\sum_{i=1}^n \hat x_i>b^*\opt(I)$, so
$\sum_{i=1}^n x_i>b^*\opt(I)$, contradicting the fact that none of the
$b$ bins in $P^*$ is packed to a level exceeding $\opt(I)$.\qed


